Creating an AI Observer: Generative Semantic Workspaces

An experienced human Observer reading a document -- such as a crime report -- creates a succinct plot-like $\textit{``Working Memory''}$ comprising different actors, their prototypical roles and states at any point, their evolution over time based on their interactions, and even a map of missing Semantic parts anticipating them in the future. $\textit{An equivalent AI Observer currently does not exist}$. We introduce the $\textbf{[G]}$enerative $\textbf{[S]}$emantic $\textbf{[W]}$orkspace (GSW) -- comprising an $\textit{``Operator''}$ and a $\textit{``Reconciler''}$ -- that leverages advancements in LLMs to create a generative-style Semantic framework, as opposed to a traditionally predefined set of lexicon labels. Given a text segment $C_n$ that describes an ongoing situation, the $\textit{Operator}$ instantiates actor-centric Semantic maps (termed ``Workspace instance'' $\mathcal{W}_n$). The $\textit{Reconciler}$ resolves differences between $\mathcal{W}_n$ and a ``Working memory'' $\mathcal{M}_n^*$ to generate the updated $\mathcal{M}_{n+1}^*$. GSW outperforms well-known baselines on several tasks ($\sim 94\%$ vs. FST, GLEN, BertSRL - multi-sentence Semantics extraction, $\sim 15\%$ vs. NLI-BERT, $\sim 35\%$ vs. QA). By mirroring the real Observer, GSW provides the first step towards Spatial Computing assistants capable of understanding individual intentions and predicting future behavior.

==> Tables/FST_output.tex <==
% Frame: Building_subparts
% Building_part: complex

% Frame: Containing
% Container: the complex
% Contents: the artesia police department, eddy county sheriff ’s office, artesia fire department, artesia municipal court, new mexico state police and the new mexico probation and parole

% Frame: Locale_by_use
% Locale: complex

% Frame: Ordinal_numbers
% Type: police shooting reported in artesia in about a month

% Frame: Killing
% Killer: police

% Frame: Statement
% Message: he fired at them during a foot chase on sept. 28 in an alley near dallas and 7th streets
% Place: in artesia
% Speaker: police

% Frame: Calendric_unit
% Unit: month

% Frame: Relative_time
% Focal_occasion: brandon sevier, 23, was shot and injured
% Landmark_occasion: police said he fired at them during a foot chase on sept. 28 in an alley near dallas and 7th streets

% Frame: Hit_target
% Target: brandon sevier, 23
% Time: after police said he fired at them during a foot chase on sept. 28 in an alley near dallas and 7th streets

% Frame: Cause_harm
% Victim: brandon sevier, 23
% Time: after police said he fired at them during a foot chase on sept. 28 in an alley near dallas and 7th streets

% Frame: Shoot_projectiles
% Agent: he
% Goal: at them
% Time: during a foot chase on sept. 28 in an alley near dallas and 7th streets

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}l@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Frame: Building\_subparts\\ Building\_part: complex\end{tabular}                                                                                                                                                                                          \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Containing\\ Container: the complex\\ Contents: the artesia police department, eddy county sheriff ’s office, \\ artesia fire department, artesia municipal court, new mexico state \\ police and the new mexico probation and parole\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Locale\_by\_use\\ Locale: complex\end{tabular}                                                                                                                                                                                                     \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Ordinal\_numbers\\ Type: police shooting reported in artesia in about a month\end{tabular}                                                                                                                                                         \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Killing\\ Killer: police\end{tabular}                                                                                                                                                                                                              \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Statement\\ Message: he fired at them during a foot chase on sept. 28 in an alley \\ near dallas and 7th streets\\ Place: in artesia\\ Speaker: police\end{tabular}                                                                                \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Calendric\_unit\\ Unit: month\end{tabular}                                                                                                                                                                                                         \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Relative\_time\\ Focal\_occasion: brandon sevier, 23, was shot and injured\\ Landmark\_occasion: police said he fired at them during a foot chase \\ on sept. 28 in an alley near dallas and 7th streets\end{tabular}                              \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Hit\_target\\ Target: brandon sevier, 23\\ Time: after police said he fired at them during a foot chase on sept. 28\\ in an alley near dallas and 7th streets\end{tabular}                                                                         \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Cause\_harm\\ Victim: brandon sevier, 23\\ Time: after police said he fired at them during a foot chase on sept. 28 \\ in an alley near dallas and 7th streets\end{tabular}                                                                        \\ \midrule
\begin{tabular}[c]{@{}l@{}}Frame: Shoot\_projectiles\\ Agent: he\\ Goal: at them\\ Time: during a foot chase on sept. 28 in an alley near dallas and 7th \\ streets\end{tabular}                                                                                                     \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/SRL_output.tex <==
% verb: reopened
% object, thing affected: the complex

% verb: was
% object, thing affected: this
% instrument, benefactive, attribute: the second police shooting reported in artesia in about a month , after brandon sevier , 23 , was shot and injured after police said he fired at them during a foot chase on sept . 28 in an alley near dallas and 7th streets

% verb: reported
% object, thing affected: the second police shooting

% verb: shot
% object, thing affected: brandon sevier , 23 ,

% verb: injured
% object, thing affected: brandon sevier , 23 ,

% verb: said
% agent: police
% object, thing affected: he fired at them during a foot chase on sept . 28 in an alley near dallas and 7th streets

% verb: fired
% agent: he


% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]
\begin{tabular}{@{}l@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: reopened\\ \textbf{object, thing affected}: the complex\end{tabular}                                                                                                                                                                                                                                                                     \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: was\\ \textbf{object, thing affected}: this\\ \textbf{instrument, benefactive, attribute}: the second police\\ shooting reported in artesia in about a month , after \\ brandon sevier , 23 , was shot and injured after police \\ said he fired at them during a foot chase on sept . 28 in \\ an alley near dallas and 7th streets\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: reported\\ \textbf{object, thing affected}: the second police shooting\end{tabular}                                                                                                                                                                                                                                                      \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: shot\\ \textbf{object, thing affected}: brandon sevier , 23 ,\end{tabular}                                                                                                                                                                                                                                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: injured\\ \textbf{object, thing affected}: brandon sevier , 23 ,\end{tabular}                                                                                                                                                                                                                                                            \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: said\\ agent: police\\ \textbf{object, thing affected}: he fired at them during a foot \\ chase on sept . 28 in an alley near dallas and 7th streets\end{tabular}                                                                                                                                                                        \\ \midrule
\begin{tabular}[c]{@{}l@{}}\textbf{verb}: fired\\ \textbf{agent}: he\end{tabular}                                                                                                                                                                                                                                                                                                  \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/comparison.tex <==
\begin{table}[h]
\resizebox{\columnwidth}{!}{%
\begin{tabular}{@{}l|l|l|l|l@{}}
\toprule
\multicolumn{1}{l|}{\textbf{Ours}} & \textbf{SRL} & \textbf{VerbNet} & \textbf{ConceptNet} & \textbf{FrameNet} \\ \midrule
\multicolumn{5}{c}{\textbf{Workspace Instance}} \\ \midrule
\multicolumn{1}{l|}{Situation} & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & Frame \\ \midrule
\multicolumn{1}{l|}{Actor} & NP / NNP & NP / NNP & Concept & \begin{tabular}[c]{@{}l@{}}(part of)\\ Lexical Units\end{tabular} \\ \midrule
\multicolumn{1}{l|}{Role} & Role & Role & \cellcolor[HTML]{EFEFEF}- & Frame Element \\ \midrule
\multicolumn{1}{l|}{State} & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \begin{tabular}[c]{@{}l@{}}*Precedence\\ Relationships\end{tabular} \\ \midrule
\multicolumn{1}{l|}{Question} & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- \\ \midrule
\multicolumn{1}{l|}{Predicate} & \cellcolor[HTML]{EFEFEF}- & \cellcolor[HTML]{EFEFEF}- & \begin{tabular}[c]{@{}l@{}}common-sense\\ relationships\end{tabular} & \begin{tabular}[c]{@{}l@{}}(part of)\\ Lexical Units\end{tabular} \\ \midrule
\multicolumn{5}{c}{\textbf{Schema Construction}} \\ \midrule
\multicolumn{1}{l|}{Open Schema} & \multicolumn{4}{c}{Fixed Schema} \\ \midrule
\multicolumn{1}{l|}{Self-supervised} & \multicolumn{4}{c}{Supervised} \\ \bottomrule
\end{tabular}%
}
\caption{\textbf{Unifying the existing semantic representation modeling terminology with the proposed Workspace model:} Semantic units in the workspace model can be mapped to existing semantic representation model units. We list the similarities and differences in this table.}
\label{tab:sandd}
\end{table}

==> Tables/glen_output.tex <==
% Event: housing
% Description: construction and assignment of houses or buildings for sheltering people
% trigger_words: ['houses']

% Event: closure
% Description: actions taken when it is no longer necessary or possible for a business or other organization to continue to operate
% trigger_words: ['reopened']

% Event: shooting
% Description: act or process of firing firearms or other projectile weapons
% trigger_words: ['shot', 'shooting']

% Event: reporting
% Description: producing a report (oral or written)
% trigger_words: ['reported']

% Event: chase
% Description: activity where one party tries to catch the other, esp. as subject in art and literature
% trigger_words: ['chase']

% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[]

% \renewcommand{\arraystretch}{0.6} % Default value: 1
% \addtolength{\tabcolsep}{-3.5pt}
\small 

\begin{tabular}{@{}l@{}}
\toprule
\begin{tabular}[c]{@{}l@{}}Event: housing\\ Description: construction and assignment of houses or buildings for sheltering people\\ trigger\_words: {[}'houses'{]}\end{tabular}                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}Event: closure\\ Description: actions taken when it is no longer necessary or possible for a business or other organization to continue to operate\\ trigger\_words: {[}'reopened'{]}\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Event: shooting\\ Description: act or process of firing firearms or other projectile weapons\\ trigger\_words: {[}'shot', 'shooting'{]}\end{tabular}                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}Event: reporting\\ Description: producing a report (oral or written)\\ trigger\_words: {[}'reported'{]}\end{tabular}                                                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}Event: chase\\ Description: activity where one party tries to catch the other, esp. as subject in art and literature\\ trigger\_words: {[}'chase'{]}\end{tabular}                                  \\ \bottomrule
\end{tabular}
\end{table}

==> Tables/operator_output.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{booktabs}
\begin{table}[h!]
\centering \small
\begin{tabular}{@{}l|l|l@{}}
\toprule
\textbf{Agents in the situation}                                                                                           & \textbf{Interactions}                                                                                                                         & \textbf{What to think about next}                                                                                                                                                                                                                                       \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: artesia municipal court\\ Role: justice administration\\ State: active\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Source: the complex\\ Interaction: houses\\ Target: artesia municipal court\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}What is the relationship between \\ the artesia police department, eddy \\ county sheriff’s office, artesia fire \\ department, artesia municipal court, \\ new mexico state police and the \\ new mexico probation and parole?\end{tabular} \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: the complex\\ Role: crime scene\\ State: investigated\end{tabular}                       & \begin{tabular}[c]{@{}l@{}}Source: the complex\\ Interaction: houses\\ Target: new mexico state police\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Where is the artesia police \\ department located in the complex?\end{tabular}                                                                                                                                                               \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: new mexico state police\\ Role: investigation\\ State: active\end{tabular}               & \begin{tabular}[c]{@{}l@{}}Source: the complex\\ Interaction: houses\\ Target: artesia fire department\end{tabular}                           & \begin{tabular}[c]{@{}l@{}}Who are the artesia police department, \\ eddy county sheriff’s office, artesia \\ fire department, artesia municipal \\ court, new mexico state police and the\\ new mexico probation and parole?\end{tabular}                              \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: police\\ Role: shooter\\ State: active\end{tabular}                                      & \begin{tabular}[c]{@{}l@{}}Source: the complex\\ Interaction: houses\\ Target: eddy county sheriff’s office\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}How did the artesia police department \\ and new mexico probation and parole \\ respond to the incident involving \\ brandon sevier?\end{tabular}                                                                                            \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: artesia fire department\\ Role: emergency response\\ State: on standby\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Source: new mexico state police\\ Interaction: investigated at\\ Target: the complex\end{tabular}                  & \begin{tabular}[c]{@{}l@{}}When was the first police shooting\\ reported in artesia?\end{tabular}                                                                                                                                                                       \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: eddy county sheriff’s office\\ Role: law enforcement\\ State: investigating\end{tabular} & \begin{tabular}[c]{@{}l@{}}Source: new mexico state police\\ Interaction: investigated shooting of\\ Target: brandon sevier\end{tabular}      & \begin{tabular}[c]{@{}l@{}}Why was the complex reopened at 8 a.m. \\ on friday?\end{tabular}                                                                                                                                                                            \\ \midrule
\begin{tabular}[c]{@{}l@{}}Agent: brandon sevier\\ Role: shooting victim\\ State: injured\end{tabular}                     & \begin{tabular}[c]{@{}l@{}}Source: police\\ Interaction: uses as base\\ Target: the complex\end{tabular}                                      &                                                                                                                                                                                                                                                                         \\ \midrule
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Source: police\\ Interaction: shot at\\ Target: brandon sevier\end{tabular}                                        &                                                                                                                                                                                                                                                                         \\ \midrule
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Source: eddy county sheriff’s office\\ Interaction: uses as headquarters\\ Target: the complex\end{tabular}        &                                                                                                                                                                                                                                                                         \\ \midrule
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Source: eddy county sheriff’s office\\ Interaction: investigated shooting of\\ Target: brandon sevier\end{tabular} &                                                                                                                                                                                                                                                                         \\ \midrule
                                                                                                                           & \begin{tabular}[c]{@{}l@{}}Source: brandon sevier\\ Interaction: fired at\\ Target: police\end{tabular}                                       &                                                                                                                                                                                                                                                                         \\ \bottomrule
\end{tabular}
\end{table}

==> extras.tex <==






such as PropBank~\cite{propbank}, Verbnet~\cite{verbnet}, and FrameNet~\cite{framenet}. In these, the \textit{space itself} (corresponding to our definition of a \textit{Workspace}) is usually delineated into an \textit{prescribed} set of \textit{explicit},  \textit{hierarchically-ordered, discrete and finite categories}, see for example, the (original) Propbank ontology (\textit{simplified}):
\begin{center}
\small
Verb (predicate) $\leftarrow$ \textbf{Frame} $\rightarrow$ Semantic Roles
\end{center}

or the FrameNet ontology (\textit{simplified}):

\begin{center}
\small
Super Frames \\
$\downarrow$ \\
Lexical Units (LU) $\leftarrow$ \textbf{Frames} $\rightarrow$ Frame Elements (FE) \\
                    $\downarrow$ \\
                Precedence Relationships to other Frames
\end{center}

% The collection of these categories~\cite{} -- and more specifically the category \textit{labels}, requires expert annotations~\cite{}, including label \textit{definitions}~\cite{}.

The population of these ontology facets yields a rich database of semantic descriptors. For example, the \textit{Committing Crime} frame in FrameNet has the following organization:

\begin{center}
\small
Misdeed (Frame) \\
$\downarrow$ \\
perpetrate.v, crime.n $\leftarrow$ \textbf{Committing Crime} $\rightarrow$ Perpetrator, Crime, ... \\
                    $\downarrow$ \\
                Precedes: Criminal Investigation (Frame)
\end{center}

or the \textit{Bringing} frame:

\begin{center}
\small
None \\
$\downarrow$ \\
bring.v, haul.v, ... $\leftarrow$ \textbf{Bringing} $\rightarrow$ Agent, Area, Carrier, ... \\
                    $\downarrow$ \\
                Precedes: Criminal Investigation (Frame)
\end{center}





The explicit, finite set of labels employed by existing ontologies results in a coarse semantic structure. For example, under FrameNet, the sentence "Officers captured Sarah at the Sepulveda on-ramp 199
of the 405" can be understood as occurring within the Frame Crime and Justice with frame elements... The explicit definition of Frames and constituent frame elements constrains the ontology to modelling semantics at a coarser level, as enumerating frames to describe finer levels of detail becomes unfeasible. 

While the construction of the Workspace The only way to evaluate the resulting workspace definition in a real-world application is \textit{to learn a model} that maps any given text input onto this semantic space: we have already defined the term \textit{Workspace Model}. 

Given the discrete and finite workspace definition, existing semantic representation models




: \textit{despite constructing the ontology, the categories themselves are difficult to interpret for a non-linguist}.



``frames'' in FrameNet for ,  corresponding to different semantic facets and attributes. For example, Propbank (applied via BertSRL) describes the sentence 
\begin{center}
    Officers captured Sarah at the Sepulveda on-ramp of the 405.
\end{center}
Agent: Officers, Predicate: captured, Patient: Sarah. 
Under Propbank, semantics are tied to explicit predicates in text, and a fixed list of 5 argument-roles (agent, patient, etc.) describe how actors interact. While Propbank has been widely used, its limited set of argument roles means that it is difficult to specify fine-grained semantic differences between contexts. FrameNet attempts to address this by providing a large number of expert annotated frames and frame-elements which describe the semantics of specific scenarios. FrameNet (applied via FrameSemanticTransformer) describes the previous sentence as:
Frame: Leadership
Leader: Officers
Frame: Taking\_captive
Agent: Officers
Captive: Sarah
Place: at the Sepulveda on-ramp of the 405. 
The structure of frames and consituent frame-elements allows FrameNet to more precisely describe a variety of situations, but the fact that it is a fixed schema means, that this set of situations is limited. Furthermore, the expert annotation required to produce new frames and frame elements makes extending framenet to new situations difficult. 
 .ConceptNet operates over the space of commonsense "concepts". In all these cases, the ontology can be considered a workspace where words from a vocabulary are mapped to the semantic facets described by the ontology. Furthermore, models which attempt to annotate text based on a particular ontology, such as Frame Semantic Transformer, BertSRL, or GLEN can be considered limited workspace instance estimators, which estimate the relevant semantic facets for a limited context, often just a single sentence. 

Existing ontologies face many limitations when used as workspace models. Propbank, FrameNet, and VerbNet all make use of fixed schemas which makes it difficult to extend these ontologies to novel situations. Furthermore, these ontologies are often constructed by manual annotation of large datasets - a labor intensive process. Finally, the semantics of these ontologies are tied to occurences of a predicate in text. This makes it difficult to apply these ontologies in cases where the semantics are implied (without the use of an indicator verb) -- for example,
\begin{center}
    \textit{John Doe} was rolling in the grave.
\end{center}
-- here the semantics aren't available based solely on the verb \textit{rolling}, the \textit{intended} meaning that John \textit{would have been} upset \textit{if he were alive} is implicit in the text.

More recent efforts build upon existing ontologies to provide semantics for novel or higher-order situations. Schema Induction ~\cite{manlingli_future,manlingli_connecting_dots,event_schema_induction_by_prompting_and_verification} attempts to generate schemas for novel situations given a training dataset. The generated schemas are often specified in a semi-supervised manner, with a human controller providing a set of key words to loosely constrain the types of situations to generate schemas for. Schema inductions methods often use existing ontologies and attempt to overcome the limitations of their fixed schemas by combining elements from the ontology in a network structure to generate novel schemas. 

However, while schema induction methods allow a greater range of semantic understanding than fixed-schema ontologies, these methods require aggregating a large volume of text in order to identify and extract schemas. As a result, they applying them to single documents or limited contexts produces poor results and any schemas they produce cannot be localized to a particular context span. Furthermore, the schemas produced are fixed to a set of input documents, they cannot dynamically update the schema as the relevant context changes. 

In contrast to these existing methods, we propose a dynamic and open-domain workspace model which can describe the semantic structure of novel situations and updates it's workspace instance as contexts change. We leverage advances in LLMs to etxtract semantic structure implicit in a context, without relying on explicit tags such as indicator verbs. Furthermore, this workspace not only represents the semantic content of a particular context, it predicts likely future states the model will observe.










Owing to the inherent complexity, syntactic nuances and polysemy of language, the semantics are often implicit. For example, a sentence as simple as,
\begin{center}
\textit{John Doe} was \textit{caught} in the morning. 
\end{center}
implies to a \textit{human} reader that,
\begin{center}2
``John Doe'' is likely a reference to a \textit{person}, \\
``caught'' refers to \textit{running} from or \textit{escaping} something.
\end{center}
A human reader might additionally ask targeted information-seeking questions that they hope will be resolved in the future: 
\begin{center}
``What was John running from?'', \\
``What happened next to John?''. 
\end{center}

The ability to estimate these hidden and implicit \textit{semantic representations} is critical to gaining a better understanding of the real generative model underlying language creation~\cite{,,}; Indeed, this goal and subproblems constitute among the longest running and challenging tasks in NLP: the \textit{latent} semantics are, by definition, \textit{hidden} and the \textit{observables} (generated text samples), are \textit{noisy}. 

Comprehensive lens through which knowledge understanding can be done:
Who where what when how

Workspace comes in generative  sense. What might happen.
Workspace need to build memory such that new parts will fit in at any time, open valences


Era of LLMs and embeddings
some kind of enumeration of verbs
fixed schema databases are actually useless

Intuitional division distributions
Distributions

Small size LLMs are not very good at showing the similarities but ChatGPT can. 

Conscious-
All bias is knowledge.
LoRA is adding in the bias.


ChatGPT has the basic connections
LoRAs 

Pruning 




In many works, the semantic representation space is manually constructed with expert annotators identifying the dominant and recurrent semantics shared over large-scale text data. For example, \david Current frameworks (to construct an ontology of semantic parts) such as FrameNet, PropBank, VerbNet, ConceptNet (for more, see Related Works~\cite{sec:related}) -- though very much works-in-progress -- have demonstrated overwhelming utility in deeper language comprehension~\cite{blah,,} and targeted information retrieval~\cite{blah,,}. Despite this, serious challenges remain. To a large extent, current methods: \david


\begin{itemize}
    \item[A] Require human annotation and curation to construct the explicit semantic ontologies~\cite{blah}. This results in challenges with schema completeness and quality of the annotations. Some annotation schemes can be so challenging that downstream models that are tasked with mapping new text segments onto these ontologies require several million training parameters and examples. For example, \david
    
    \item[B] Do not have a sense of \textit{prioritization}: Some semantics are more important than others. Models constructed to map text onto these semantics usually iterate through ALL the verbs (more generally, \textit{predicates}) in the input text, and use these as ``anchors'' or starting points to detect semantics -- whether this semantic facet is ``important'' or not. For example, 
\end{itemize}














{\color{red} A  few succinct sentences describing the task and what we mean by situational awareness, Draw inspiration from: Frames as Mental Structures: A frame is a cognitive structure of knowledge that arises during our interaction with the world and other people. It's like a mental schema or a script that helps us understand and interpret a variety of situations and linguistic expressions. For instance, the "restaurant frame" includes knowledge about what a restaurant is, the roles (e.g., customer, waiter), actions (e.g., ordering, eating), and objects (e.g., menu, table) involved in a dining experience.}

{\color{red} A  couple of succinct sentences about the existing NLP works, such as FrameNet, SRL, event detection,  which have tried to solve this proble:} Automated extraction of situational models expressed in text has been an important NLP task \cite{}. Traditionally, it has been framed as a suervised task, where the first step is to define a hierarchical ontology of situations comprising ...... 





In this paper, we unify the several pre-existing motivations for constructing semantic representation spaces\footnote{Moreover, many of these existing frameworks were developed far before Large Language Models (LLM), and it remains to be seen whether the development of LLMs can facilitate a more general or powerful workspace construction.}, by first and foremost, noting that the need to construct semantic representations is supported by cutting-edge neuroscientific advances and pathological evidence of a \textit{dedicated} region in the Neocortex, termed the \textit{``Global Workspace''} that is key to \textit{human} semantic reasoning capabilities across various sensory modalities~\cite{blah,,}.

Accordingly, we (a) present a novel and inclusive formalism and computational model of a ``Workspace'', and reorient existing semantics estimation paradigms into this view. Following this, we (b) demonstrate a powerful self-supervised method (and implementation) to estimate the  parameters of the \textit{Workspace model} -- an \textit{inverse} problem given large-scale text data. Last, we demonstrate some early downstream applications of such a model in constructing workspace instances and language generation. An overview is presented in Fig.~\ref{fig:overview}. 

% Researchers have hypothesized that these semantics are  and that language is merely an observable signal generated from and assimilated into this semantics layer~\cite{blah,,}. While similar semantic abilities may arise implicitly within Large Language models (LLMs), such abilities are difficult to verify and directly manipulate. Instead, explicitly modelling this semantic workspace provides a concrete path towards equipping LLMs with deeper language understanding. 













  % In the longer term, the construction of a Workspace promises to facilitate efficient and prioritized memory architectures for long-term planning and \textit{controlled and semantically guardrailed} generation tasks~\cite{,,}. 

% ---

% This paper reviews existing workspace models in NLP and proposes a modernized alternative that is better suited for the world of LLMs and generative modeling. Among the key differences,  As we will see later, such a setup offers several advantages including a potentially infinite workspace ontology that results in the construction of a richer semantics space.




% , since for any situation, such as ``\textit{Going to the Supermarket}'' or ``\textit{Visiting the dentist}'', one can learn a dedicated set of parameters.




% \subsection{Essential Characteristics of a Workspace Instance}

% Workspace instances, due to limitations in computational capacity and the real-time demands of learning, must adhere to the following fundamental requirements:

% \begin{enumerate}


% \item[\textbf{R1}] \textit{Compositional Capacity:} Workspaces must possess the ability to represent an infinite array of intricate situations. This necessitates constructing a finite set of building blocks that can be combined in diverse ways to articulate various circumstances.

% % Grey shaded box for R1

% \item[\textbf{R2}] \textit{Predictive Capability:} Just as biological workspaces excel at task completion~\cite{blah,,}, workspace instances should possess inherent predictive abilities. They should adeptly identify missing elements within a partially completed workspace and strategize to acquire them. Additionally, these workspaces need to foresee potential future circumstances and reason about them effectively.

% \item[\textbf{R3}] \textit{Dynamic Adaptability:} Workspace instances are inherently dynamic, continually evolving as new contexts emerge. They must undergo constant modifications to maintain an up-to-date state in response to the presentation of new information or scenarios.

% \end{enumerate}









% % put later.
% FrameNet annotations also include a sparse set of temporal relationships between the frames: \textit{preceded by}, \textit{precedes}, \textit{caused by}, \textit{causes}. For example, the \{crime\} frame \textit{precedes} the \{arrest\} frame and this, in turn precedes \{arraignment\}. 


% \noindent \textbf{SemLink:} 

% \noindent \textbf{ConceptNet}: ConceptNet~\cite{conceptnet} provides a dataset of commonsense concepts and relationships derived from both crowd-sourced and expert-annotated work. These concepts are organized in a network, where semantically related concepts are linked. 

% \noindent \textbf{ACE}: The Automatic Content Extraction (ACE) ~\cite{ACE} program sought to develop methods for the extraction of entities, relations, and events from text data. To this end,  the program developed ACE2005, a multilingual dataset which provides annotations for several types of entities, relations, and events. 



% \color{red}
% \section{Background}

% Recent models have shown to excel at producing language using a generative architecture~\cite{blah,,,}. In creative applications, a prior context (or \textit{prompt}) $C_1, \dots, C_{N-1}$ is typically input into an (implicit)  function $f$ with parameters $\theta$ such that,
% $$
% f_{\theta}(C_1, \dots, C_{N-1})
% $$
% is a distribution. When contexts are exploitatively (greedy) or exploratively (higher temperature) sampled in a recursive fashion, $f$ produces a string of $K$ new contexts, $C_N, \dots,C_{N+K}$ -- an autoregressive use-case. Today, such models have demonstrated success at such impressive usecases as LSAT / GRE examinations, interview coding tests, and copy-editing across writing tasks~\cite{blah,,}.

% Despite these models' achievements, generating data that \textit{is specific to} the user's requirements is significantly more challenging~\cite{gan,,} -- known as the \textit{planning problem}~\cite{plan,,}. Generative applications are exponentially more viable, and indeed safe, if the outputs are \textit{guardrailed} syntactically and semantically~\cite{blah,,}. Solutions are being actively researched: Recently, \textit{prompt engineering}~\cite{blah,,} argues that users wrest back creative control (or \textit{plan}) by iteratively manipulating the input $C_1, \dots, C_{N-1}$ to shape the output distribution. 

% Such shotgun methods have however proven to be fickle~\cite{blah,,} and painstaking~\cite{blah,,}, and are to be rediscovered and reformulated for every new model checkpoint~\cite{blah,,}. To make matters worse, existing generative models are shown to perform better at limited context lengths (N): Even if the user did painstakingly write and tune a prompt, how can we guarantee that the model would remain sensitive to the \textit{entire} instructions, and not \textit{ignore} a few critical parts? Despite recent models boasting longer context lengths, they are still, at the very least, more expensive (by computation cost, and dollar cost-per-token). 

% In this work, we introduce an alternate perspective and early evidence to address such challenges in Large-Scale Language Models (LLM), termed \textit{Situation Modeling}. 

% \begin{definition}
% Situation: A prototype or recurring theme in stories and activities observed in real-life; for example, "driving to the supermarket", "flying to another country", "development of technology" etc.
% \end{definition}


% \begin{definition}
% Situation models: Self-supervised models that construct and maintain \textit{atomic}, \textit{interpretable}, and \textit{extendable} representations of stereotypical themes constituting a situation.
% \end{definition}
% \color{black}








% \subsubsection{Situation Models}
% \noindent \textbf{Downstream Models:} Several research efforts have attempted to create models that utilize the previously discussed ontologies to classify novel text spans. Among those utilizing FrameNet \cite{open-sesame, framenet-transformer}, models typically consist of rule-based and deep architectures that classify \textit{any} input text into frames (via lexical unit matching for instance), and then attribute FE tags to specific text spans within the context. Several works attempt to utilize the ACE2005 dataset to perform entity, relation, and event extraction from text. The most succesful ~\cite{oneie, dygie} have applied transformer models such as BERT to encode input text and classify spans as entity, relation, or event. These spans are then added to internal graph structures in order to ensure consistent annotations. 

% ~\cite{bert-srl}



==> formulation.tex <==




% \begin{figure}
%     \centering
%     \includegraphics[width=\columnwidth]{Figures/schema.pdf}
%     \caption{\textbf{Overview of the node and edge types in a Workspace instance:} An Actor embodies a set of Roles within a specific context at any given time, navigating and influencing other Actors (and their respective Roles and States) using Predicates. Leading questions are also added as valences to the instance in the hope that a future input text context will resolve these missing attributes.}
%     \label{fig:schema}
% \end{figure}

% \definecolor{lightgray}{RGB}{240,240,240} % Define a light grey color

% \begin{center}
%     \colorbox{lightgray}{\parbox{0.99\linewidth}{
%         \noindent \textbf{Actor} \\ A noun phrase that features in a Situation; \\
%         \textbf{Role} \\ \textit{Archetypal descriptors}, shaping an Actor's predisposition within a Situation; \\
%         \textbf{State} \\ \textit{Dynamic descriptors} that define the current \textit{valence} of a Role, influencing potential relationships between Roles at any given moment; \\
%         \textbf{Predicate} \\ Interactions between Actors. \\
%         \textbf{Question} \\ \textit{Predictive valences} that anticipate what role-state / predicate is next, given the active nodes, edges; 
%     }}
% \end{center}



\section{Data}

News reports are a popular resource for sampling semantics-rich stories that belong to universally-recognized situation patterns (in an effort to cater to a wider readership). We query GDELT~\cite{gdelt}, a Jigsaw-powered news-indexing platform and parse the resulting articles with BeautifulSoup~\cite{bs4}.  Tab.~\ref{tab:data} presents statistics about the data. These situations were manually selected as an initial seed set -- similar to FrameNet's first few frames~\cite{fillmore} -- to assess the validity of the framework since they have a large number of correponding lexicon identifiers in Event and Frame databases. A separate Operator-Reconciler pair is trained for each situation to begin with. However, we will later show that the situation-to-situation generalization of the trained models is strong (Sec.~\ref{sec:ablation}): I.e. we may not need to learn a separate model for each situation.

\input{Tables/data_content}



% \section{Operator: Semantics as a Conditional Random Field} \label{sec:distributions}

% The task of the Operator is to \textit{learn a distribution over the lexicon} given an overarching situation. Given an input context $C_i$, the Operator estimates the following conditional distributions: \textbf{Roles} are conditioned on the input text segment and a specific \textbf{actor} $a$ identified in the context: $r \sim P(\cdot | C_i, a)$ - \textit{different actors would occupy different roles}. Given an actor $a$ assuming role $r$, the \textbf{state} is then estimated as: $s \sim P(\cdot | C_i, a, r)$ - \textit{actors in different roles will take on different subsets of states}. Finally, a futuristic \textbf{question} $q$ is sampled from a distribution given the text segment: $q \sim P(\cdot | C_i)$ and \textbf{predicates} between source actor $a_S$ and target actor $a_T$ pairs are estimated: $p \sim P(\cdot | C_i, a_S, a_T)$.

% \begin{tcolorbox}[colback=mycolor,colframe=black,width=\dimexpr1.0\columnwidth\relax]
% \small
%     \textbf{Theorem 1}
%     A workspace instance $\mathcal{W}_i$ can be computationally modeled as a complex network $\mathcal{W}_i(V,E)$. A formal probabilistic intepretation is presented in the Sec.~\ref{app:probabilistic} (see Fig.~\ref{fig:spotlight}, Sec.~\ref{app:sec:examples} for sample networks).
% \end{tcolorbox}



% The task of the Operator is to \textit{learn a distribution over the lexicon} given an overarching situation. Given an input context $C_i$, the Operator estimates the following conditional distributions: \textbf{Roles} are estimated as conditioned on the input text segment and the specific \textbf{actor} $a$ identified in the context: $r \sim P(\cdot | C_i, a)$: \textit{different actors would occupy different roles}. Conditioned on the actor $a$ and its assumed role $r$, the \textbf{state} is then estimated as: $s \sim P(\cdot | C_i, a, r)$: \textit{an actor can only be in a subset of }\textbf{states} \textit{when it inhabits a specific role}. Similarly, a futuristic \textbf{question} $q$ is sampled from a distribution given the text segment: $q \sim P(\cdot | C_i)$. \textbf{Predicates} between pairs of source actor $a_S$ and target actor $a_T$ are estimated last: $p \sim P(\cdot | C_i, a_S, a_T)$.



\subsection{Training Details} 

We utilize a \textit{teacher-student} approach (see Fig.~\ref{fig:distributed}): (1) First, a GPT-4~\cite{gpt4} ``teacher'' model directed by Guidance\footnote{ \small \url{github.com/guidance-ai/guidance}} generates workspace instances in an open-end creative task (for the prompt, please see our codebase\footnote{\small \url{anonymous.4open.science/r/OperatorNet}}). The Guidance prompt ($>1000$ tokens) uses expert-annotated prompt tricks~\cite{prompt} to encourage GPT-4 to act as an expert linguist and generate \textit{stereotypical} lexicon \textit{instances} of the roles, states, predicates, and questions identified in a corpus of short context $C_i$. Where needed, the prompt also encourages the generation of  \textit{negative} samples (which output the ``None'' default lexicon) to discourage spurious roles and inter-actor predicates. (2) We use parameter-efficient fine-tuning (PeFT)~\cite{prefixtuning,llamaadapter} to train a LLaMA-2~\cite{llama2} ``student'' model. Different QLoRA~\cite{qlora} adapters are learned for each situation and can be inserted into the LLaMA backbone to match situation-specific input contexts (plug-and-play).  Each adapter contains ~1M parameters (rank-2) and requires very few samples (80) to train. 

% Features of the Operator models, the label data collection, and training methodology are provided below (see Fig.~\ref{fig:distributed}):
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Teacher-Student Model:} First, workspace instances are generated in an open-end creative task using GPT-4~\cite{gpt4} and Guidance\footnote{\url{https://github.com/guidance-ai/guidance}} (see our codebase\footnote{\url{https://anonymous.4open.science/r/OperatorNet/}}). 
%     % Can maybe fold this into the above sentence
%     \color{red}This \color{black} forms the ``teacher''-backbone; 
%     \item \textbf{Parameter-efficient Fine-tuning:} The ``student'' model uses a Llama-2~\cite{llama2} architecture and a small subset of parameters are learned: (PeFT) QLoRA-adapter~\cite{llamaadapter, qlora, prefixtuning}. Each PeFT adapter contains ~1M parameters (rank-2) and requires few samples to train. Different adapters can be inserted into the LLaMA backbone for different situations (plug-and-play);
%     \item \textbf{Prompt Engineering:} The Guidance prompt ($>1000$ tokens) uses expert-motivated prompt engineering findings~\cite{prompt} to encourage GPT-4 to behave as an expert linguist and generate \textit{stereotypical} lexicon instances of the roles, states, predicates, questions identified in a short context $C_i$. Where needed, the prompt also encourages the generation of  \textit{negative} samples (to output the ``None'' default lexicon) which encourages the student model to avoid generating spurious roles and inter-actor predicates.
% \end{itemize}


\begin{figure}[h]
    \centering
\includegraphics[width=0.8\columnwidth]{Figures/distributed.pdf}
    \caption{\textbf{Modular parameter sets for the Workspace model:} Every Operator and Reconciler model (specific to a situation) comprises $<1M$ parameters -- using PeFT and LoRA -- and relies on the same shared LLM Oracle (LLaMA-2-13B). }
    \label{fig:distributed}
\end{figure}




% \section{A Probabilistic Interpretation of a Workspace Instance as a Complex Network} \label{app:probabilistic}

% One can view the task of jointly estimating a workspace instance as the estimation of a \textit{complex network}:
% $$\mathcal{W}:=\mathcal{W}(V,E),$$ 
% where the nodes $v \in V$ and edges $e \in E$ correspond to the following lexicon map:

% \noindent \textbf{Node:} \{Actor, Role, State\}; \{Question\}\\
% \noindent \textbf{Edge:} Source Actor $\rightarrow$ Predicate $\rightarrow$ Target Actor.
% \\

% \noindent Then, the workspace instance itself can be viewed as a sample generated by the Operator:
% \begin{align*}
% \mathcal{W} \sim g_{\Phi}(C_i) \implies V_{\mathcal{W}_i}, E_{\mathcal{W}_i} \sim g_{\Phi}(C_i).
% \end{align*}
% Assume conditional independence: 
% $$P(V_{\mathcal{W}_i}, E_{\mathcal{W}_i} | C_i) \approx \prod P(\{v_S, e, v_T\} | C_i).$$ 
% \begin{align*}
% P(\{v_S, e&, v_T\} | C_i) = \\&P(e | v_S, v_T, C_i) \times P(v_S, v_T | C_i).
% \end{align*}

% Now, $P(v_S, v_T | C_i) = P(v_S| C_i) \times P(v_T| C_i)$. Each can be further decomposed:
% \begin{align*}
% P(v | C_i) &:= P(\{a, r, s\} | C_i) \\
% &= P(s | a, r; C_i) \\ &  \times P(r | a; C_i) \times P(a | C_i)
% \end{align*}
% Therefore, the set of conditional lexicon distributions learned by the Operator are sufficient to describe the likelihood of generating the entire workspace instance as a complex network.


% \noindent \textbf{Why Complex Networks?} Complex networks are a suitable representation for a semantic map construction -- akin to the Frame hierarchy observed in FrameNet or the concept graph assembled in ConceptNet -- owing to its (a) atomic nature in representing the individual parts of the lexicon, as well as (b) the ability to selectively retrieve subnetworks that correspond to a subset of actors and their current states. We will use these advantages while modeling the \textit{Reconciler} in the next section.







\section{Reconciler: Similarity across Workspace Instances}

The Reconciler computes the similarity between the workspace instance -- now modeled as a Complex Network (see Sec.~\ref{app:probabilistic}) -- already populating the workspace and the latest Operator-generated instance $\mathcal{W}_i$ (recall Fig.~\ref{fig:overview}).

The Reconciler has three choices: (i) Keep what is currently in the workspace instance and discard the new information (as noise or infeasible); (ii) Discard specific lexical parts in the workspace instance and repopulate with parts of the new Operator output; (iii) Keep both the existing lexicon samples as well as the new Operator-generated lexicon samples since they do not conflict. The Reconciler is thus posed as a \textit{classifier} (see Tab.~\ref{tab:reconciler-labels}) and uses the same model architecture as the Operator.

\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{0.30em} % Adjust the column separation here
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Reconciler Classification Labels}}                                                                                                                                                                                                                                    \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Nodes, \\Edges\end{tabular}} & \begin{tabular}[c]{@{}l@{}}0: the existing workspace instance is sufficient\\ 1: the new instance overwrites the workspace\\ 2: both instances are important and unrelated\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Questions\end{tabular}}      & \begin{tabular}[c]{@{}l@{}}0: question remains unanswered and relevant\\ 1: question is answered or irrelevant\end{tabular}                                                             \\ \bottomrule
\end{tabular}
\caption{\textbf{Summary of classification tasks trained in the Reconciler:} Nodes and edges are classified pairwise -- \textit{Reconciliation} or REC -- into one of three classes (0: keep previous, 1: replace, 2: keep both), and \{question, node\} and \{question, edge\} pairs are classified -- \textit{Question Resolution} or QR -- as answered or irrelevant (1) or unanswered and relevant (0).}
\label{tab:reconciler-labels}
\end{table}


% \subsection{Training Details} 
% Given a sequence of input contexts $C_1, \dots, C_N$, the Reconciler is trained to resolve conflicting lexicon and remove outdated parts. In addition to silver-standard classification labels on the true data, we \textit{generate} synthetic lexicon instances from GPT-4 as a \textit{bootstrapping} technique to ensure a balanced training dataset across classes. Classification examples are presented as pairs of nodes and edges, where one is from the pre-existing workspace instance and the other is from the Operator output instance. Since the workspace instance is often substantially larger than the latest Operator output instance, the Reconciler only infers on a subgraph in the workspace (identified using a naive similarity measure and a Retrieval method~\cite{retrieval}) that is likely to change given the latest information. 

% The Reconciler model training methodology and training dataset collections details are provided below:
% \begin{itemize}[leftmargin=*]
%     \item \textbf{Streaming:} Given a sequence of input contexts $C_1, \dots, C_N$, the Reconciler is trained to resolve conflicting lexicon and remove outdated parts. In addition to silver-standard classification labels on the true data, we \textit{generate} synthetic lexicon instances from GPT-4 as a bootstrapping technique to ensure a balanced training dataset;
%     \item \textbf{Retrieval:} The Reconciler is trained on pairs of nodes and edges where one half is from the existing workspace instance and the other half is from the Operator output instance. Since the workspace instance is often substantially larger than the latest Operator output instance, the Reconciler only infers on a subgraph in the workspace -- identified using naive similarity measure and a Retrieval method~\cite{retrieval} -- that is likely to change given the latest information. 
% \end{itemize}

A summary overview of the various Operator and Reconciler subtasks is presented in Tab.~\ref{tab:subtasks} and a training workflow is presented in Fig.~\ref{fig:data}.

\begin{table}[h]
\small
\centering
\setlength{\tabcolsep}{1.3em} % Adjust the column separation here
\begingroup
\renewcommand{\arraystretch}{0.4} % Default value: 1
\begin{tabular}{@{}ll@{}}
\toprule
\multicolumn{2}{c}{\textbf{Summary of Subtasks}}                                                                                                                                                                         \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Operator\\ (Generation)\end{tabular}}       & \begin{tabular}[c]{@{}l@{}}Actor / Role / State Identification,\\  Question and Predicate Generation\end{tabular} \\ \midrule
\multicolumn{1}{l|}{\begin{tabular}[c]{@{}l@{}}Reconciler\\ (Classification)\end{tabular}} & \begin{tabular}[c]{@{}l@{}}Node and Edge Reconciliation, \\ Question Resolution\end{tabular}                \\ \bottomrule
\end{tabular}
\endgroup
\caption{\textbf{Summary of subtasks addressed by the Operator and Reconciler:} The Operator model is tasked with generating a network-style lexicon which the Reconciler compares to the existing workspace instance -- an aggregate of several prior Operator-generated lexicon -- and outputs a new, up-to-date instance.}
\label{tab:subtasks}
\end{table}




==> framework_comparison.tex <==
% \section{Workspace Instance Comparison}

% We present a sample of workspace instances generated by the operator and baselines described in Sec ~\ref{sec:evalmethods} from the following news report snippet: 
% \begin{center}
% \noindent \textit{The complex houses the Artesia Police Department, Eddy County sheriff’s office, Artesia Fire Department, Artesia Municipal Court, New Mexico State Police and the New Mexico Probation and Parole. The complex was reopened at 8 a.m. on Friday. This was the second police shooting reported in Artesia in about a month, after brandon sevier, 23, was shot and injured after police said he fired at them during a foot chase on Sept. 28 in an alley near Dallas and 7th streets.}
% \end{center}

% \newpage

% \newpage

% \subsection{Operator}

% \begin{figure*}[h]
%     \centering
% \includegraphics[trim={20cm 0 20cm 0},clip,width=\textwidth]{Figures/bertSRL.png}
% \end{figure*}

% \input{Tables/operator_output}

% \newpage

% \subsection {BertSRL}

% \input{Tables/SRL_output}

% \subsection {Frame Semantic Transformer}

% \input{Tables/FST_output}

% \newpage

% \subsection {GLEN}

% \input{Tables/glen_output}
